Efficient Computation of the Quantum Rate-Distortion Function

The quantum rate-distortion function plays a fundamental role in quantum information theory, however there is currently no practical algorithm which can efficiently compute this function to high accuracy for moderate channel dimensions. In this paper, we show how symmetry reduction can significantly simplify common instances of the entanglement-assisted quantum rate-distortion problems. This allows us to better understand the properties of the quantum channels which obtain the optimal rate-distortion trade-off, while also allowing for more efficient computation of the quantum rate-distortion function regardless of the numerical algorithm being used. Additionally, we propose an inexact variant of the mirror descent algorithm to compute the quantum rate-distortion function with provable sublinear convergence rates. We show how this mirror descent algorithm is related to Blahut-Arimoto and expectation-maximization methods previously used to solve similar problems in information theory. Using these techniques, we present the first numerical experiments to compute a multi-qubit quantum rate-distortion function, and show that our proposed algorithm solves faster and to higher accuracy when compared to existing methods.

==> main_results.tex <==
\begin{table}[t]
    \caption{Comparison between various algorithms to compute for the quantum rate-distortion function with entanglement fidelity distortion, at channel dimensions $n$ and distortion dual variables $\kappa$. We report the time elapsed (s) and upper bounds on the absolute optimality gap (bits) of each method. We use ``$>3600.00$'' to refer when the algorithm has not solved to the desired tolerance within an hour, and report the optimality gap of the last completed iteration at this time. We use ``Timeout'' to refer to when the algorithm has not performed any iterations within an hour. }
    \centerline{
    \begin{subtable}{1.15\textwidth}\centering
        \footnotesize
        \caption{Without symmetry reduction}
        \label{tab:no-symm}
        \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lrrrrcrcrcrc@{\extracolsep{\fill}}}
        \toprule
        \multicolumn{2}{l}{} & \multicolumn{2}{c}{MD-N} & \multicolumn{2}{c}{MD-GD} & \multicolumn{2}{c}{PDHG~\cite{he2023mirror}}      & \multicolumn{2}{c}{EM~\cite{hayashi2022bregman}} & \multicolumn{2}{c}{\textsc{CvxQuad}~\cite{fawzi2018efficient,fawzi2019semidefinite}}     \\ \cmidrule{3-4}\cmidrule{5-6}\cmidrule{7-8}\cmidrule{9-10}\cmidrule{11-12}
        $n$   &   $\kappa$               & Time & Gap & Time & Gap & Time & Gap & Time & Gap & Time & Gap \\ \midrule
        $2$                    & $1.0$   & $.19$ & $\mathbf{\num{4e-9}}$  & $.12$ & $\mathrm{\num{2e-8}}$ & $\mathbf{.11}$ & $\mathrm{\num{1e-7}}$ & $.20$ & $\mathrm{\num{2e-5}}$ & $3.00$  & $\mathrm{\num{8e-9}}$          \\
                             & $3.0$   & $.13$ & $\mathbf{\num{1e-8}}$  & $.10$ & $\mathrm{\num{2e-8}}$ & $\mathbf{.05}$ & $\mathrm{\num{2e-6}}$ & $.22$ & $\mathrm{\num{5e-5}}$ & $2.94$  & $\mathrm{\num{2e-8}}$          \\
        $8$                    & $1.0$   & $4.88$ & $\mathbf{\num{2e-8}}$  & $2.30$ & $\mathrm{\num{1e-7}}$ & $\mathbf{.84}$ & $\mathrm{\num{6e-6}}$ & $7.56$ & $\mathrm{\num{4e-5}}$ & \multicolumn{2}{c}{Out of memory}          \\
                             & $3.0$   & $\mathbf{1.12}$ & $\mathbf{\num{1e-8}}$  & $2.59$ & $\mathrm{\num{2e-8}}$ & $1.40$ & $\mathrm{\num{9e-7}}$ & $6.06$ & $\mathrm{\num{3e-5}}$ & \multicolumn{2}{c}{Out of memory}          \\
        $32$                   & $3.0$   & $>3600.00$ & $\mathbf{\num{2e-7}}$ & $\mathbf{332.16}$ & $\mathrm{\num{4e-7}}$ & $355.38$ & $\mathrm{\num{3e-5}}$ & $>3600.00$ & $\mathrm{\num{6e-3}}$ & \multicolumn{2}{c}{Out of memory} \\
                             & $5.5$   & $1321.85$ & $\mathbf{\num{1e-7}}$ & $\mathbf{631.83}$ & $\mathrm{\num{2e-7}}$ & $1500.75$ & $\mathrm{\num{5e-5}}$ & $>3600.00$ & $\mathrm{\num{4e-3}}$ & \multicolumn{2}{c}{Out of memory} \\
        $128$                  & $7.0$   & \multicolumn{2}{c}{Timeout} & \multicolumn{2}{c}{Timeout} & $\mathbf{>3600.00}$ & $\mathbf{\num{2e-1}}$ & \multicolumn{2}{c}{Timeout} & \multicolumn{2}{c}{Out of memory} \\
                             & $8.5$   & \multicolumn{2}{c}{Timeout} & \multicolumn{2}{c}{Timeout} & $\mathbf{>3600.00}$ & $\mathbf{\num{1e-1}}$ & \multicolumn{2}{c}{Timeout} & \multicolumn{2}{c}{Out of memory} \\
        $512$                  & $9.5$   & \multicolumn{2}{c}{Out of memory}  & \multicolumn{2}{c}{Out of memory} & \multicolumn{2}{c}{Out of memory} & \multicolumn{2}{c}{Out of memory} & \multicolumn{2}{c}{Out of memory} \\
         & $11.0$  & \multicolumn{2}{c}{Out of memory}  & \multicolumn{2}{c}{Out of memory} & \multicolumn{2}{c}{Out of memory} &  \multicolumn{2}{c}{Out of memory}  & \multicolumn{2}{c}{Out of memory} \\ \bottomrule
        \end{tabular*}
    \end{subtable}
    }
    
    \vspace{0.5cm}    
    \centerline{
    \begin{subtable}{1.15\textwidth}\centering
        \footnotesize
        \caption{With symmetry reduction}
        \label{tab:symm}
        \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lrrrrcrcrcrc@{\extracolsep{\fill}}}
        \toprule
        \multicolumn{2}{l}{} & \multicolumn{2}{c}{MD-N} & \multicolumn{2}{c}{MD-GD} & \multicolumn{2}{c}{PDHG~\cite{he2023mirror}}      & \multicolumn{2}{c}{EM~\cite{hayashi2022bregman}} & \multicolumn{2}{c}{\textsc{CvxQuad}~\cite{fawzi2018efficient,fawzi2019semidefinite}}     \\ \cmidrule{3-4}\cmidrule{5-6}\cmidrule{7-8}\cmidrule{9-10}\cmidrule{11-12}
        $n$   &   $\kappa$               & Time & Gap & Time & Gap & Time & Gap & Time & Gap & Time & Gap \\ \midrule
        $2$                    & $1.0$   & $.06$ & $\mathrm{\num{4e-9}}$  & $\mathbf{.05}$ & $\mathrm{\num{2e-8}}$ & $\mathbf{.05}$ & $\mathrm{\num{7e-8}}$ & $.08$ & $\mathrm{\num{2e-8}}$ & $2.89$  & $\mathbf{\num{2e-9}}$          \\
                             & $3.0$   & $.05$ & $\mathrm{\num{1e-8}}$  & $\mathbf{.04}$ & $\mathrm{\num{2e-8}}$ & $.07$ & $\mathrm{\num{7e-8}}$ & $.07$ & $\mathrm{\num{5e-5}}$ & $2.61$  & $\mathbf{\num{2e-9}}$          \\
        $8$                    & $1.0$   & $.17$ & $\mathbf{\num{7e-9}}$  & $\mathbf{.10}$ & $\mathrm{\num{1e-7}}$ & $.12$ & $\mathrm{\num{6e-6}}$ & $.53$ & $\mathrm{\num{1e-6}}$ & $454.98$  & $\mathrm{\num{2e-8}}$          \\
                             & $3.0$   & $\mathbf{.07}$ & $\mathbf{\num{4e-9}}$  & $.16$ & $\mathrm{\num{8e-9}}$ & $.19$ & $\mathrm{\num{6e-7}}$ & $.41$ & $\mathrm{\num{5e-8}}$ & $686.11$  & $\mathrm{\num{6e-8}}$          \\
        $32$                   & $3.0$   & $1.52$ & $\mathbf{\num{6e-8}}$ & $\mathbf{.45}$ & $\mathrm{\num{2e-7}}$ & $1.84$ & $\mathrm{\num{2e-5}}$ & $14.83$ & $\mathrm{\num{2e-5}}$ & \multicolumn{2}{c}{Out of memory} \\
                             & $5.5$   & $\mathbf{.32}$ & $\mathbf{\num{5e-9}}$ & $.81$ & $\mathrm{\num{6e-8}}$ & $6.51$ & $\mathrm{\num{5e-5}}$ & $17.25$ & $\mathrm{\num{5e-7}}$ & \multicolumn{2}{c}{Out of memory} \\
        $128$                  & $7.0$   & $\mathbf{14.40}$ & $\mathbf{\num{3e-8}}$ & $14.97$ & $\mathrm{\num{6e-8}}$ & $47.07$ & $\mathrm{\num{1e-4}}$ & $>3600.00$ & $\mathrm{\num{6e-6}}$ & \multicolumn{2}{c}{Out of memory} \\
                             & $8.5$   & $\mathbf{8.91}$ & $\mathbf{\num{6e-10}}$ & $16.84$ & $\mathrm{\num{7e-8}}$ & $100.55$ & $\mathrm{\num{1e-4}}$ & $>3600.00$ & $\mathrm{\num{6e-7}}$ & \multicolumn{2}{c}{Out of memory} \\
        $512$                  & $9.5$   & $2174.38$ & $\mathbf{\num{7e-8}}$  & $\mathbf{140.97}$ & $\mathrm{\num{1e-7}}$ & $1650.75$ & $\mathrm{\num{3e-4}}$ & $>3600.00$ & $\mathrm{\num{9e-5}}$ & \multicolumn{2}{c}{Out of memory} \\
        & $11.0$  & $1216.96$ & $\mathbf{\num{5e-9}}$  & $\mathbf{575.86}$ & $\mathrm{\num{1e-8}}$ & $>3600.00$ & $\mathrm{\num{5e-4}}$ &  $>3600.00$  &  $\mathrm{\num{1e-4}}$  & \multicolumn{2}{c}{Out of memory} \\ \bottomrule
        \end{tabular*}
     \end{subtable}
     }
\end{table}
